Neural Network Compression using Binarization and Few Full-Precision Weights

Quantization and pruning are two effective Deep Neural Networks model compression methods. In this paper, we propose Automatic Prune Binarization (APB), a novel compression technique combining quantization with pruning. APB enhances the representational capability of binary networks using a few full-precision weights. Our technique jointly maximizes the accuracy of the network while minimizing its memory impact by deciding whether each weight should be binarized or kept in full precision. We show how to efficiently perform a forward pass through layers compressed using APB by decomposing it into a binary and a sparse-dense matrix multiplication. Moreover, we design two novel efficient algorithms for extremely quantized matrix multiplication on CPU, leveraging highly efficient bitwise operations. The proposed algorithms are 6.9x and 1.5x faster than available state-of-the-art solutions. We extensively evaluate APB on two widely adopted model compression datasets, namely CIFAR10 and ImageNet. APB delivers better accuracy/memory trade-off compared to state-of-the-art methods based on i) quantization, ii) pruning, and iii) combination of pruning and quantization. APB outperforms quantization in the accuracy/efficiency trade-off, being up to 2x faster than the 2-bit quantized model with no loss in accuracy.

==> makefile <==
### Makefile for LaTeX under Mac OS X
### Author: Franco Maria Nardini (francomaria.nardini@isti.cnr.it)
# pdflatex, textmate, and skim are needed to run properly all the commands here.

# Some assumptions:
# ./img: is the directory containing images
# ./style: is the directory containing the .cls and .sty

# NAME OF THE MAIN FILE (WITHOUT .tex)
BASEFILENAME=paper

# NAME OF THE CAMERA READY FILE (WITHOUT .pdf)
DESTFILENAME=

# NAME OF THE COVER LETTER FILE (WITHOUT .pdf)
COVERFILENAME=cover_letter


#NAME OF THE REVIEW ANSWER FILE (WITHOUT .pdf)

all:
	@make clean
	@make pdf
	@make pdf-coverletter
	@open -F -a skim ${BASEFILENAME}.pdf &
	

pdf:
	@pdflatex ${BASEFILENAME}.tex
	@bibtex ${BASEFILENAME}
	@pdflatex ${BASEFILENAME}.tex
	@pdflatex ${BASEFILENAME}.tex

	

pdf-cameraready:
	@pdflatex ${BASEFILENAME}.tex
	@pdflatex ${BASEFILENAME}.tex
	@mv ${BASEFILENAME}.pdf ${DESTFILENAME}.pdf
	@open -F -a skim ${DESTFILENAME}.pdf

pdf-coverletter:
	@pdflatex ${COVERFILENAME}.tex
	@bibtex ${BASEFILENAME}
	@pdflatex ${COVERFILENAME}.tex
	@pdflatex ${COVERFILENAME}.tex
	@rm ${COVERFILENAME}.aux
	@rm ${COVERFILENAME}.log
	@open -F -a skim ${COVERFILENAME}.pdf


answer:
	@pdflatex ${REVIEWANSWER}.tex
	@bibtex ${REVIEWANSWER}
	@pdflatex ${REVIEWANSWER}.tex
	@pdflatex ${REVIEWANSWER}.tex
	@open -F -a skim ${REVIEWANSWER}.pdf &

images:
	@for filename in `ls ./img/*.eps`; do epstopdf $$filename; done;

count:
	@pdftotext ${BASEFILENAME}.pdf WORDS
	@wc --words WORDS
	@rm -f WORDS

clean:
	@rm -f ./img/*~ *~ *vtc *spl .*.lb *loa *aux *dvi *maf *mtc *mtc0 *log *fls *lof *lot *out *pdf *bbl *blg *ps *idx *toc *fdb_latexmk *synctex.gz *auxlock *cut *vtc *synctex* *vtc

chkrefs:
	@bibtex ${BASEFILENAME}

tgz:
	@tar -czf $(PWD)\ `date +%Y%m%d%H%M`.tar.gz *tex *tmproj *bib ./img/* ./style/*

svn-commit:
	@svn update
	@svn commit -m "`date +%Y%m%d%H%M` - FM"

svn-update:
	@svn update

git-commit-push:
	@git commit -am "`date +%Y%m%d%H%M` - FM"
	@git push origin master

git-pull:
	@git pull origin master


